Automatic Data Augmentation Selection and Parametrization in Contrastive Self-Supervised Speech Representation Learning

Contrastive learning enables learning useful audio and speech representations without ground-truth labels by maximizing the similarity between latent representations of similar signal segments. In this framework various data augmentation techniques are usually exploited to help enforce desired invariances within the learned representations, improving performance on various audio tasks thanks to more robust embeddings. Now, selecting the most relevant augmentations has proven crucial for better downstream performances. Thus, this work introduces a conditional independance-based method which allows for automatically selecting a suitable distribution on the choice of augmentations and their parametrization from a set of predefined ones, for contrastive self-supervised pre-training. This is performed with respect to a downstream task of interest, hence saving a costly hyper-parameter search. Experiments performed on two different downstream tasks validate the proposed approach showing better results than experimenting without augmentation or with baseline augmentations. We furthermore conduct a qualitative analysis of the automatically selected augmentations and their variation according to the considered final downstream dataset.

==> dulo <==
@article{Xiao2020,
author = {Xiao, Tete and Wang, Xiaolong and Efros, Alexei and Darrell, Trevor},
title = {{What Should Not Be Contrastive in Contrastive Learning}},
year = {2020}
}
@misc{rivire2020unsupervised,
    title={Unsupervised pretraining transfers well across languages},
    author={Morgane Rivière and Armand Joulin and Pierre-Emmanuel Mazaré and Emmanuel Dupoux},
    year={2020},
    eprint={2002.02848},
    archivePrefix={arXiv},
    primaryClass={eess.AS}
}


@article{Nagrani_2017,
   title={VoxCeleb: A Large-Scale Speaker Identification Dataset},
   DOI={10.21437/interspeech.2017-950},
   journal={Interspeech 2017},
   publisher={ISCA},
   author={Nagrani, Arsha and Chung, Joon Son and Zisserman, Andrew},
   year={2017},
   month={Aug}
}

@misc{arcface,
  doi = {10.48550/ARXIV.1801.07698},
  
  url = {https://arxiv.org/abs/1801.07698},
  
  author = {Deng, Jiankang and Guo, Jia and Xue, Niannan and Zafeiriou, Stefanos},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {ArcFace: Additive Angular Margin Loss for Deep Face Recognition},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@article{efficientnet,
  doi = {10.48550/ARXIV.1905.11946},
  
  url = {https://arxiv.org/abs/1905.11946},
  
  author = {Tan, Mingxing and Le, Quoc V.},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {EfficientNet: Rethinking Model Scaling for Convolutional Neural Networks},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@inproceedings{Zaiem_2021,
	doi = {10.21437/interspeech.2021-1027},
  
	url = {https://doi.org/10.21437%2Finterspeech.2021-1027},
  
	year = 2021,
	month = {aug},
  
	publisher = {{ISCA}
},
  
	author = {Salah Zaiem and Titouan Parcollet and Slim Essid},
  
	title = {Conditional Independence for Pretext Task Selection in Self-Supervised Speech Representation Learning},
  
	booktitle = {Interspeech 2021}
}
@misc{https://doi.org/10.48550/arxiv.2107.00594,
  doi = {10.48550/ARXIV.2107.00594},
  
  url = {https://arxiv.org/abs/2107.00594},
  
  author = {Zaiem, Salah and Parcollet, Titouan and Essid, Slim},
  
  keywords = {Audio and Speech Processing (eess.AS), Machine Learning (cs.LG), Sound (cs.SD), Machine Learning (stat.ML), FOS: Electrical engineering, electronic engineering, information engineering, FOS: Electrical engineering, electronic engineering, information engineering, FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Pretext Tasks selection for multitask self-supervised speech representation learning},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{Arora2019,
abstract = {Recent empirit controlled experiments in both the text and image domains to support the theory.},
annote = {The number of negative samples has been an important point to take into account in contrastive algorithms. Increasing highly this number may lead to class collisions even if the number of NS is much smaller than the number of classes.
If we consider that similar points are elements of the same class, then, making their embeddings closer should help if the downstream task is a classification one on a subset of these classes.},
archivePrefix = {arXiv},
arxivId = {1902.09229},
author = {Arora, Sanjeev and Khandeparkar, Hrishikesh and Khodak, Mikhail and Plevrakis, Orestis and Saunshi, Nikunj},
eprint = {1902.09229},
file = {:home/salah/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Arora et al. - 2019 - A Theoretical Analysis of Contrastive Unsupervised Representation Learning.pdf:pdf},
journal = {36th International Conference on Machine Learning, ICML 2019},
mendeley-groups = {Unsupervised Representation learning},
month = {feb},
pages = {9904--9923},
publisher = {International Machine Learning Society (IMLS)},
title = {{A Theoretical Analysis of Contrastive Unsupervised Representation Learning}},
volume = {2019-June},
year = {2019}
}

@inproceedings{Shor_2020,
	doi = {10.21437/interspeech.2020-1242},
  
	url = {https://doi.org/10.21437%2Finterspeech.2020-1242},
  
	year = 2020,
	month = {oct},
  
	publisher = {{ISCA}
},
  
	author = {Joel Shor and Aren Jansen and Ronnie Maor and Oran Lang and Omry Tuval and F{\'{e}}lix de Chaumont Quitry and Marco Tagliasacchi and Ira Shavitt and Dotan Emanuel and Yinnon Haviv},
  
	title = {Towards Learning a Universal Non-Semantic Representation of Speech},
  
	booktitle = {Interspeech 2020}
}

@misc{baevski2020wav2vec,
      title={wav2vec 2.0: A Framework for Self-Supervised Learning of Speech Representations}, 
      author={Alexei Baevski and Henry Zhou and Abdelrahman Mohamed and Michael Auli},
      year={2020},
      eprint={2006.11477},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}
@article{Liu_2020,
   title={Mockingjay: Unsupervised Speech Representation Learning with Deep Bidirectional Transformer Encoders},
   ISBN={9781509066315},
   DOI={10.1109/icassp40776.2020.9054458},
   journal={ICASSP 2020 - 2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
   publisher={IEEE},
   author={Liu, Andy T. and Yang, Shu-wen and Chi, Po-Han and Hsu, Po-chun and Lee, Hung-yi},
   year={2020},
   month={May}
}

@misc{ardila2020common,
      title={Common Voice: A Massively-Multilingual Speech Corpus}, 
      author={Rosana Ardila and Megan Branson and Kelly Davis and Michael Henretty and Michael Kohler and Josh Meyer and Reuben Morais and Lindsay Saunders and Francis M. Tyers and Gregor Weber},
      year={2020},
      eprint={1912.06670},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}
@misc{lee2020predicting,
      title={Predicting What You Already Know Helps: Provable Self-Supervised Learning}, 
      author={Jason D. Lee and Qi Lei and Nikunj Saunshi and Jiacheng Zhuo},
      year={2020},
      eprint={2008.01064},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}
@misc{zaiem,
  doi = {10.48550/ARXIV.2107.00594},
  
  url = {https://arxiv.org/abs/2107.00594},
  
  author = {Zaiem, Salah and Parcollet, Titouan and Essid, Slim},
  
  keywords = {Audio and Speech Processing (eess.AS), Machine Learning (cs.LG), Sound (cs.SD), Machine Learning (stat.ML), FOS: Electrical engineering, electronic engineering, information engineering, FOS: Electrical engineering, electronic engineering, information engineering, FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Pretext Tasks selection for multitask self-supervised speech representation learning},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}
@techreport{Wang,
abstract = {Recent advances suggest the advantage of multi-modal training in comparison with single-modal methods. In contrast to this view, in our work we find that similar gain can be obtained from training with different formats of a single modality. In particular, we investigate the use of the contrastive learning framework to learn audio representations by maximizing the agreement between the raw audio and its spectral representation. We find a significant gain using this multi-format strategy against the single-format counterparts. Moreover, on the downstream AudioSet and ESC-50 classification task, our audio-only approach achieves new state-of-the-art results with a mean average precision of 0.376 and an accuracy of 90.5%, respectively.},
archivePrefix = {arXiv},
arxivId = {2103.06508v3},
author = {Wang, Luyu and Deepmind, Google},
eprint = {2103.06508v3},
file = {::},
mendeley-groups = {Unsupervised Speech Learning},
title = {{Multi-Format Contrastive Learning of Audio Representations}}
}



@misc{speechbrain,
  title={SpeechBrain: A General-Purpose Speech Toolkit},
  author={Mirco Ravanelli and Titouan Parcollet and Peter Plantinga and Aku Rouhe and Samuele Cornell and Loren Lugosch and Cem Subakan and Nauman Dawalatabad and Abdelwahab Heba and Jianyuan Zhong and Ju-Chieh Chou and Sung-Lin Yeh and Szu-Wei Fu and Chien-Feng Liao and Elena Rastorgueva and François Grondin and William Aris and Hwidong Na and Yan Gao and Renato De Mori and Yoshua Bengio},
  year={2021},
  eprint={2106.04624},
  archivePrefix={arXiv},
  primaryClass={eess.AS}
}
@misc{byol,
  doi = {10.48550/ARXIV.2006.07733},
  
  url = {https://arxiv.org/abs/2006.07733},
  
  author = {Grill, Jean-Bastien and Strub, Florian and Altché, Florent and Tallec, Corentin and Richemond, Pierre H. and Buchatskaya, Elena and Doersch, Carl and Pires, Bernardo Avila and Guo, Zhaohan Daniel and Azar, Mohammad Gheshlaghi and Piot, Bilal and Kavukcuoglu, Koray and Munos, Rémi and Valko, Michal},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Bootstrap your own latent: A new approach to self-supervised Learning},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{simclr,
  doi = {10.48550/ARXIV.2002.05709},
  
  url = {https://arxiv.org/abs/2002.05709},
  
  author = {Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {A Simple Framework for Contrastive Learning of Visual Representations},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@INPROCEEDINGS{kharitonov,

  author={Kharitonov, Eugene and Rivière, Morgane and Synnaeve, Gabriel and Wolf, Lior and Mazaré, Pierre-Emmanuel and Douze, Matthijs and Dupoux, Emmanuel},

  booktitle={2021 IEEE Spoken Language Technology Workshop (SLT)}, 

  title={Data Augmenting Contrastive Learning of Speech Representations in the Time Domain}, 

  year={2021},

  volume={},

  number={},

  pages={215-222},

  doi={10.1109/SLT48900.2021.9383605}}

@misc{cola,
  doi = {10.48550/ARXIV.2010.10915},
  
  url = {https://arxiv.org/abs/2010.10915},
  
  author = {Saeed, Aaqib and Grangier, David and Zeghidour, Neil},
  
  keywords = {Sound (cs.SD), Machine Learning (cs.LG), Audio and Speech Processing (eess.AS), FOS: Computer and information sciences, FOS: Computer and information sciences, FOS: Electrical engineering, electronic engineering, information engineering, FOS: Electrical engineering, electronic engineering, information engineering},
  
  title = {Contrastive Learning of General-Purpose Audio Representations},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}
@article{Emami2021,
abstract = {Impsound/event classification tasks.},
archivePrefix = {arXiv},
arxivId = {2112.10950},
author = {Emami, Melikasadat and Tran, Dung and Koishida, Kazuhito},
eprint = {2112.10950},
file = {::},
keywords = {Index Terms-self-supervised learning,audio data augmentation,contrastive learning,feature invariance},
mendeley-groups = {Unsupervised Speech Learning},
month = {dec},
title = {{Augmented Contrastive Self-Supervised Learning for Audio Invariant Representations}},
url = {http://arxiv.org/abs/2112.10950},
year = {2021}
}

@inproceedings{maclean2018voxforge,
  title={Voxforge},
  author={MacLean, Ken},
  journal={Ken MacLean.[Online]. Available: http://www.voxforge.org/home.[Acedido em 2012]},
  year={2018}
}
@misc{shor2021,
  doi = {10.48550/ARXIV.2110.04621},
  
  url = {https://arxiv.org/abs/2110.04621},
  
  author = {Shor, Joel and Jansen, Aren and Han, Wei and Park, Daniel and Zhang, Yu},
  
  keywords = {Sound (cs.SD), Machine Learning (cs.LG), Audio and Speech Processing (eess.AS), FOS: Computer and information sciences, FOS: Computer and information sciences, FOS: Electrical engineering, electronic engineering, information engineering, FOS: Electrical engineering, electronic engineering, information engineering},
  
  title = {Universal Paralinguistic Speech Representations Using Self-Supervised Conformers},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {Creative Commons Attribution 4.0 International}
}
@techreport{Al-Tahan2021,
abstract = {Learning rich visual representations using contrastive self-supervised learning has been extremely  1 .},
author = {Al-Tahan, Haider and Mohsenzadeh, Yalda},
file = {:home/salah/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Al-Tahan, Mohsenzadeh - 2021 - CLAR Contrastive Learning of Auditory Representations.pdf:pdf},
mendeley-groups = {Unsupervised Speech Learning},
title = {{CLAR: Contrastive Learning of Auditory Representations}},
url = {https://github.com/},
year = {2021}
}

@article{tian2020makes,
  abstract = {Contrastive learning between multiple views of the data has recently achieved
classification ($73\%$ top-1 linear readoff with a ResNet-50). In addition,
transferring our models to PASCAL VOC object detection and COCO instance
segmentation consistently outperforms supervised pre-training.
Code:http://github.com/HobbitLong/PyContrast},
  added-at = {2020-05-22T03:15:16.000+0200},
  author = {Tian, Yonglong and Sun, Chen and Poole, Ben and Krishnan, Dilip and Schmid, Cordelia and Isola, Phillip},
  biburl = {https://www.bibsonomy.org/bibtex/239d42b4bf50e9cbb754b2ee9e745417c/kirk86},
  description = {[2005.10243] What makes for good views for contrastive learning},
  interhash = {cf3646ea3019b06404681616039a3e1e},
  intrahash = {39d42b4bf50e9cbb754b2ee9e745417c},
  keywords = {bayesian mutual-information readings unsupervised},
  note = {cite arxiv:2005.10243Comment: submitted to ECCV 2020},
  timestamp = {2020-05-22T03:15:16.000+0200},
  title = {What makes for good views for contrastive learning},
  url = {http://arxiv.org/abs/2005.10243},
  year = 2020
}


==> out.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green01270}{RGB}{0,127,0}

\begin{groupplot}[group style={group size=2 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={Language ID},
x grid style={darkgray176},
xmin=-0.475, xmax=4.475,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={bandreject,pitch,reverb,time\_drop,clip},
y grid style={darkgray176},
ymin=-0.208527531074899, ymax=0.225862548157444,
ytick style={color=black}
]
\draw[draw=none,fill=green01270] (axis cs:0.75,0) rectangle (axis cs:1.25,0.184049957109641);
\draw[draw=none,fill=green01270] (axis cs:1.75,0) rectangle (axis cs:2.25,0.0902786280197447);
\draw[draw=none,fill=green01270] (axis cs:3.75,0) rectangle (axis cs:4.25,0.132989939735951);
\draw[draw=none,fill=red] (axis cs:-0.25,0) rectangle (axis cs:0.25,-0.0612691028187037);
\draw[draw=none,fill=red] (axis cs:2.75,0) rectangle (axis cs:3.25,-0.019693863922605);

\nextgroupplot[
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
title={Speaker ID},
x grid style={darkgray176},
xmin=-0.475, xmax=4.475,
xtick style={color=black},
xtick={0,1,2,3,4},
xticklabels={bandreject,pitch,reverb,time\_drop,clip},
y grid style={darkgray176},
ymin=-0.208527531074899, ymax=0.225862548157444,
ytick style={color=black},
yticklabels={}
]
\draw[draw=none,fill=green01270] (axis cs:0.75,0) rectangle (axis cs:1.25,0.206117544555974);
\draw[draw=none,fill=green01270] (axis cs:2.75,0) rectangle (axis cs:3.25,0.0632253552074544);
\draw[draw=none,fill=red] (axis cs:-0.25,0) rectangle (axis cs:0.25,-0.0429262939609826);
\draw[draw=none,fill=red] (axis cs:1.75,0) rectangle (axis cs:2.25,-0.0729764421020777);
\draw[draw=none,fill=red] (axis cs:3.75,0) rectangle (axis cs:4.25,-0.188782527473428);
\end{groupplot}

\end{tikzpicture}

